Taste or Strategy? Nationalistic Bias and Competitor Penalties in Figure Skating Judging

Many decisions rest on expert panels whose members have ties to some candidates, and favoritism is hard to tell from shared taste or better information. Using a rich dataset from figure skating, we find evidence of a strategic compatriot premium and a targeted penalty on the compatriot's close rivals. The premium falls along a randomly drawn start order and, before 2022/23, rises when close rivals have their own judges on the panel. The penalty grows with the compatriot's placement chances and fades once she is out of contention. A counterfactual analysis shows that these biases can shape close competitions.

==> tables/table_A_D_3_continued.tex <==
\begin{tabular}{lrrrrrr}
\toprule
 & \multicolumn{3}{c}{\textbf{All rows}} & \multicolumn{3}{c}{\textbf{Championships and Olympics}} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
\textbf{Variable} & \textbf{(4) TSS pct} & \textbf{(5) GOE pct} & \textbf{(6) PCS pct} & \textbf{(7) TSS pct} & \textbf{(8) GOE pct} & \textbf{(9) PCS pct} \\
\midrule
Prior Worlds placement & +2.757*** & +1.993** & +3.213*** & +0.949 & -0.691 & +1.478** \\
 & (0.741) & (0.760) & (0.548) & (0.832) & (1.027) & (0.637) \\
Prior Worlds best place (0 if none) & -0.062** & -0.004 & -0.076*** & +0.009 & +0.102** & -0.008 \\
 & (0.030) & (0.032) & (0.022) & (0.033) & (0.043) & (0.023) \\
Prior World Juniors placement & +1.346*** & +0.395 & +1.919*** & +0.365 & -0.970 & +1.087** \\
 & (0.456) & (0.530) & (0.351) & (0.807) & (0.956) & (0.466) \\
Prior World Juniors best place (0 if none) & -0.017 & +0.006 & -0.037** & +0.033 & +0.032 & -0.018 \\
 & (0.021) & (0.024) & (0.015) & (0.036) & (0.050) & (0.021) \\
First season in junior events & -1.778*** & -1.466*** & -1.589*** & -0.278 & -0.808 & -0.301 \\
 & (0.472) & (0.501) & (0.352) & (0.898) & (1.080) & (0.599) \\
First season in senior events & -0.451 & +0.197 & -0.540 & -0.036 & +0.654 & -0.174 \\
 & (0.525) & (0.596) & (0.432) & (0.578) & (0.789) & (0.375) \\
Music: film & +0.284* & +0.235 & +0.222*** & +0.240 & +0.390 & +0.159 \\
 & (0.147) & (0.223) & (0.084) & (0.274) & (0.324) & (0.172) \\
Music: stage & +0.344 & +0.380 & +0.306* & +0.734 & +1.181** & +0.587** \\
 & (0.250) & (0.297) & (0.167) & (0.444) & (0.554) & (0.253) \\
Music: classical & +0.319 & +0.280 & +0.246 & +0.166 & +0.403 & +0.201 \\
 & (0.230) & (0.297) & (0.154) & (0.292) & (0.453) & (0.166) \\
Music: opera & -0.044 & +0.148 & +0.145 & +0.019 & -0.047 & +0.133 \\
 & (0.360) & (0.518) & (0.190) & (0.812) & (1.164) & (0.308) \\
Music: contemporary instrumental & +0.144 & +0.391 & +0.131 & +0.415 & +0.475 & +0.242 \\
 & (0.221) & (0.265) & (0.139) & (0.317) & (0.351) & (0.157) \\
Music: others & -0.016 & +0.086 & -0.016 & +0.669 & +1.719 & +0.512 \\
 & (0.474) & (0.685) & (0.306) & (0.710) & (1.083) & (0.471) \\
Music: mixed & +0.151 & +0.030 & +0.138 & +0.254 & -0.082 & +0.241 \\
 & (0.154) & (0.214) & (0.103) & (0.255) & (0.298) & (0.146) \\
$\mathrm{Start}_{p}$ & +3.863*** & +1.450*** & +5.562*** & +8.353*** & +4.545*** & +10.809*** \\
 & (0.330) & (0.416) & (0.310) & (0.671) & (0.924) & (0.501) \\
\midrule
The 30 choreographer indicators (shown apart) & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
Compatriot, Rival, Other-panel compatriot, Home ice, the technical panel & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
Compatriot $\times$ home ice & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
Other-segment compatriot &  &  &  & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
Skater FE & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
Segment FE & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
Judge FE & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
N & 206,983 & 206,983 & 206,983 & 55,276 & 55,276 & 55,276 \\
\# of Competitions (G) & 172 & 172 & 172 & 30 & 30 & 30 \\
\# of Federations (F) & 78 & 78 & 78 & 60 & 60 & 60 \\
\bottomrule
\end{tabular}

